Fixed-PSNR Lossy Compression for Scientific Data

Error-controlled lossy compression has been studied for years because of extremely large volumes of data being produced by today's scientific simulations. None of existing lossy compressors, however, allow users to fix the peak signal-to-noise ratio (PSNR) during compression, although PSNR has been considered as one of the most significant indicators to assess compression quality. In this paper, we propose a novel technique providing a fixed-PSNR lossy compression for scientific data sets. We implement our proposed method based on the SZ lossy compression framework and release the code as an open-source toolkit. We evaluate our fixed-PSNR compressor on three real-world high-performance computing data sets. Experiments show that our solution has a high accuracy in controlling PSNR, with an average deviation of 0.1 ~ 5.0 dB on the tested data sets.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> tex/lossy.tex <==
\section{Lossy Checkpointing Scheme for Iterative Methods}
\label{sec:lossy}

In this section, we first analyze the expected overhead of checkpointing techniques for iterative methods. 
We prove that reducing the checkpointing overhead (e.g., by leveraging compression techniques) can significantly improve the overall performance, especially for future HPC systems.
This analysis motivates us to design an approach to reduce the checkpointing overhead.
Then, we propose our lossy checkpointing scheme that can be easily applied to iterative methods in numerical linear algebra.
We also present a new performance model for our lossy checkpointing scheme. Based on the model, we derive an upper bound for the number of extra iterations caused by lossy checkpoints against the reduced checkpointing overhead, in order to guarantee the performance improvement of the lossy checkpointing scheme.
We theoretically and empirically analyze the impact of lossy checkpointing on the convergence of iterative methods considering multiple types of iterative methods.
%\vspace{-1mm}

\subsection{Theoretical Analysis of Checkpointing Overhead for Iterative Methods}
If a failure happens, we restart the computation from the last checkpointed variables, as shown in Algorithm 2. 
This process is normally called \textit{rollback}. 
Rollback means that some previous computations need to be performed again.
Thus, the checkpointing frequency or time interval needs to be determined carefully.
Here the checkpointing interval is the mean time between two checkpoints.
On the one hand, a larger checkpointing interval means a longer rollback in case of failure, indicating more workload to be recomputed after the recovery;
on the other hand, a smaller checkpointing interval means more frequent checkpointing, leading to higher checkpointing overhead.
How to calculate the optimal checkpointing intervals has been studied for many years \cite{young, agbaria1999starfish}.
Our following analysis is based on the recovery pattern of iterative methods constructed by Langou et al. \cite{langou}. 

% \begin{table}[]
% \centering
% \caption{My caption}
% \label{my-label}
% \begin{tabular}{|l|l|}
% \hline
% $T_{it}$            & Mean time of an iteration                                                                                           \\ \hline
% $T_{ckp}$           & Mean time to perform a checkpoint                                                                                   \\ \hline
% $T_{rc}$            & \begin{tabular}[c]{@{}l@{}}Mean time to recover the application from\\ the last checkpoint\end{tabular}             \\ \hline
% $T_{rb}$            & Mean time to perform a rollback                                                                                     \\ \hline
% $T_f$               & Mean time to failure (MTTF)                                                                                         \\ \hline
% $T_{overhead}^{CR}$ & Mean time overhead of checkpoint/recovery                                                                           \\ \hline
% $\lambda$           & Failure rate, i.e, 1/$T_f$                                                                                          \\ \hline
% $k$                 & \begin{tabular}[c]{@{}l@{}}The checkpoint frequency - a checkpoint is performed\\ every $k$ iterations\end{tabular} \\ \hline
% $N$                 & Number of iterations to converge without failures                                                                   \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[]
\centering
\caption{Notation for traditional checkpointing model}
%\vspace{-2mm}
\label{tab:notation}
\resizebox{\hsize}{!}{%
\begin{tabular}{|l|l|}
\hline
$T_{it}$  & Mean time of an iteration                                                                                       \\ \hline
$T_{ckp}$ & Mean time to perform a checkpoint                                                                             \\ \hline
$T_{rc}$  & \begin{tabular}[c]{@{}l@{}}Mean time to recover the application with the correct \\ environment and data from the last checkpoint\end{tabular}        \\ \hline

$T_{rb}$  & \begin{tabular}[c]{@{}l@{}}Mean time to perform a rollback of some redundant \\  computations\end{tabular}                                                                        \\ \hline
$T_f$     & Mean time to interruption                                                                                     \\ \hline
$T_{overhead}^{CR}$     & Mean time overhead of checkpoint/recovery                                                                                     \\ \hline
$\lambda$ & Failure rate, i.e, 1/$T_f$                                                                                      \\ \hline
$k$       & \begin{tabular}[c]{@{}l@{}}Checkpoint frequency - a checkpoint is performed\\ every $k$ iterations\end{tabular} \\ \hline
$N$       & Number of iterations to converge without failures                                                               \\ \hline
\end{tabular}
}
%\vspace{-3mm}
\end{table}

We use the notation in Table \ref{tab:notation} to analyze the expected fault tolerance overhead.
The overall execution time $T_t$ can be expressed as 
\begin{equation*}
\vspace{-0.5mm}
T_{t} = NT_{it} + T_{ckp}\frac{N}{k} + \frac{T_{t}}{T_{f}}(T_{rc} + T_{rb}).
\vspace{-0.5mm}
\end{equation*}

Without loss of generality, based on Young's formula \cite{young}, the optimal checkpointing interval should be chosen as 
\begin{equation}
\label{eq:young}
\vspace{-0.5mm}
k\cdot T_{it} = \sqrt{2T_{f}\cdot T_{ckp}}, 
\vspace{-0.5mm}
\end{equation}
and the expected mean time to perform a roll back, namely, $T_{rb}$, is $kT_{it}/2$. 
Thus,
\begin{align*}
\vspace{-1mm}
T_{t} &= NT_{it} + T_{ckp}\frac{T_{t}}{\sqrt{2T_{f}\cdot T_{ckp}}} + \frac{T_{t}}{T_{f}}(T_{rc} + \frac{\sqrt{2T_{f}\cdot T_{ckp}}}{2}) \\
%	&= NT_{it} + T_{t}(\frac{T_{ckp}}{\sqrt{2T_{f}\cdot T_{ckp}}} + \frac{T_{rc}}{T_f} + \frac{\sqrt{2T_{f}\cdot T_{ckp}}}{2T_f}) \\
%	&= NT_{it} + T_{t}(\sqrt{\frac{T_{ckp}}{2T_f}} + \frac{T_{rc}}{T_f} + \sqrt{\frac{T_{ckp}}{2T_f}}) \\
	&= NT_{it} + T_{t}(\sqrt{\frac{2T_{ckp}}{T_f}} + \frac{T_{rc}}{T_f}) = NT_{it} + T_{t}(\sqrt{2\lambda T_{ckp}} + \lambda T_{rc}).
\vspace{-0.5mm}
\end{align*}

Similar to \cite{langou}, we therefore can get the expected overall execution time as 
\begin{equation}
\vspace{-0.5mm}
T_{t} = \frac{NT_{it}}{1 - \sqrt{2\lambda T_{ckp}} - \lambda T_{rc}},
\vspace{-0.3mm}
\end{equation}
and the fault tolerance overhead is 
\begin{equation}
\vspace{-0.3mm}
T_{overhead}^{CR} = T_{t} - NT_{it} = NT_{it}\cdot \frac{\sqrt{2\lambda T_{ckp}} + \lambda T_{rc}}{1 - \sqrt{2\lambda T_{ckp}} - \lambda T_{rc}},
\vspace{-0.3mm}
\end{equation}
where $NT_{it}$ is the basic productive execution time with $N$ iterations to converge. Note that here we use \textit{fault tolerance overhead} to refer to the performance overhead caused by checkpoints/recoveries and failure events, which is equal to the total running time taking away the basic productive execution time (i.e., $T_t$$-$$N$$T_{it}$).

We assume $T_{rc} \approx T_{ckp}$ without loss of generality. Then we can simplify the expected fault tolerance overhead as follows.
\begin{equation}
\label{eq:lossless-overhead}
\vspace{-0.5mm}
T_{overhead}^{CR} \approx NT_{it}\cdot \frac{\sqrt{2\lambda T_{ckp}} + \lambda T_{ckp}}{1 - \sqrt{2\lambda T_{ckp}} - \lambda T_{ckp}}
\vspace{-0.5mm}
\end{equation}
Moreover, we can calculate the ratio of the expected fault tolerance overhead to the basic productive execution time as Equation (\ref{eq:Toverhead}).
\begin{equation}
\label{eq:Toverhead}
\frac{T_{overhead}^{CR}}{NT_{it}} = \frac{\sqrt{2\lambda T_{ckp}} + \lambda T_{ckp}}{1 - \sqrt{2\lambda T_{ckp}} - \lambda T_{ckp}}
\end{equation}

\begin{figure}[t]
\centering
\includegraphics[scale=0.30]{Fig/Fig1.pdf}
\vspace{-4mm}
\caption{Expected fault tolerance overhead with different failure rates and checkpoint time.}
\vspace{-5mm}
\label{fig:f1}
\end{figure}

Now the expected fault tolerance overhead depends only on the failure rate $\lambda$ and time of one checkpoint $T_{ckp}$.
Based on this formula, we can plot the expected overhead of checkpoint/recovery based on different $\lambda$ and $T_{ckp}$, as shown in Figure \ref{fig:f1}.
We choose $\lambda$ from $0$ to $3.5$ failures per hour (i.e., MTTI from about $20$ minutes to infinity) and $T_{ckp}$ from $0$ to $140$ seconds. Note that the MTTI represents the expected period at which the application execution is interrupted.
Based on our experimental evaluation, checkpointing one dynamic vector $x$ once without compression takes about $120$ seconds with $2,048$ processes/cores on the Bebop cluster \cite{bebop} at Argonne National Laboratory.
% too far away - as shown in Table \ref{tab:size}.
%\textcolor{red}{One issue here is that 78.8GB is very small. BlueWaters has 1.5 PB of memory. So how the timings and results evolve if you consider solving PDEs filling the memory of BlueWaters, knowing that its file system peaks at 1TB/s}.
In our experiment, the number of elements in the vector is set to $10^{10}$ (with $78.8$ GB double-precision floating-point data), which is the largest problem size that the three iterative methods (Jacobi, GMRES, and CG) can be run on the Bebop using 2,048 cores. 
We adopt the FTI library \cite{fti} with MPI-IO for checkpointing because of its high I/O efficiency confirmed in recent studies \cite{mpiio}. More details are presented in the experimental evaluation section.

Figure \ref{fig:f1} illustrates that the expected fault tolerance overhead can be as high as $40\%$ with $T_{ckp} = 120s$ if the MTTI is about hourly.
On future extreme-scale systems with millions of components, the failure rate may be higher, and the fault tolerance overhead issue could be more severe.
From Figure \ref{fig:f1}, we see that reducing the checkpointing time can significantly improve the overall performance of checkpoint/restart, especially under a higher error rate scenario.
% We propose to apply state-of-the-art lossy compression approaches, such as SZ lossy compressor, to checkpointing technique for iterative methods.
% In this paper, we use \textit{lossy checkpointing} to represent the checkpointing technique with lossy compression.

\subsection{Lossy Checkpointing Scheme for Iterative Methods}
\label{sec:lossy-chkpt-scheme}
Our  lossy checkpointing scheme based on an iterative method has two key steps.
\begin{itemize}
\item Compress dynamic variables with lossy compressor before each checkpointing.
\item Decompress compressed dynamic variables after each recovering.
\end{itemize}

\begin{algorithm}[]
\caption{Fault-tolerant preconditioned conjugate gradient algorithm with lossy checkpointing technique}
\footnotesize
\begin{flushleft}
\textbf{Input:} linear system matrix $A$, preconditioner $M$, and right-hand side vector $b$\\
\textbf{Output:} approximate solution $x$
\end{flushleft}

\begin{algorithmic}[1]
\STATE Initialization: same as line 1 in Algorithm 1
\FOR{$i = 0, 1, \cdots$}
\IF {(($i > 0$) and ($i\%ckpt\_intvl = 0$))}
\STATE \textbf{Compress: $x^{(i)}$ with lossy compressor}
\STATE \textit{Checkpoint: $i$ and compressed $x^{(i)}$}
\ENDIF
\IF {(($i > 0$) and (recover))}
\STATE \textit{Recover: $A, M, i$ and compressed $x^{(i)}$}
\STATE \textbf{Decompress:  $x^{(i)}$ with lossy compressor}
\STATE Compute $r^{(i)} = b - Ax^{(i)}$
\STATE Solve $Mz^{(i)} = r^{(i)}$
\STATE $p^{(i)} = z^{(i)}$
\STATE $\rho_i = {r^{(i)}}^Tz^{(i)}$
\ENDIF
\STATE Computation: same as lines 10--17 in Algorithm 1
\ENDFOR
\end{algorithmic}
\end{algorithm}

We still use the CG algorithm as an example, as shown in Algorithm 2; and the lossy checkpointing scheme can be applied to other iterative methods similarly.
Because of space limitations, we present only the lossy checkpointing part without the original computations in Algorithm 2. 
The lossy compression and decompression procedures are marked in bold.
We note that the CG algorithm maintains a series of orthogonality relations between the residual vectors $r$ and the direction vectors $p$.
Specifically, (1) $p^{(k)}$ and $Aq^{(j)}$, (2) $r^{(k)}$ and $p^{(j)}$, and (3) $r^{(k)}$ and $r^{(j)}$ are orthogonal to each other, where $j < k$.
However, these orthogonality relations may be broken after a recovery because of the errors introduced by lossy compression.
Unfortunately, the convergence rate of the CG algorithm (which is superlinear) is highly dependent on these orthogonality relations.
Hence, after a recovery from lossy checkpointing, the CG algorithm may lose the superlinear convergence rate, leading to a slow convergence \cite{sao2013self}.
To avoid this situation, we adopt a restarted scheme for the CG algorithm (\emph{restarted CG}) \cite{powell1977restart},
% the intermediate memory is cleared from time to time and
in which the computed approximate solution $x_i$ is periodically treated as a new guess. 
%Such a revised CG is also called \emph{restarted CG}.
In this case, we need to checkpoint only the vector $x_i$ during the execution. The decompressed $x_i$ is used as a new initial guess, and a new series of orthogonal vectors is reconstructed for the execution, such that a superlinear convergence rate can be rebuilt after restart.

Some studies of iterative methods have proved that such a restarted version of iterative methods (i.e., restarting by treating the current approximate solution vector as a new initial guess) may bring important advantages \cite{powell1977restart,agullo2013towards,gmres}. 
On the one hand, it suffers from less time and space complexity compared with its classic counterparts. For example, in practice, GMRES  is often used to be restarted every a number of iterations (denoted by $k$) with the vector $x_k$ as a new initial guess; and it is often denoted by GMRES($k$).
Without the periodically restarting feature, the total time and space complexity of GMRES will both grow with an increasing rate of $N^2$ over the time step $N$.
%and its space complexity will grow with a rate of $N$.
By contrast, the time and space complexity of GMRES($k$) will be limited under a constant cost over the execution. 
On the other hand, some studies \cite{agullo2013towards,gmres} have proved that the \emph{restarted scheme} may not delay the convergence but even accelerate it, in that the periodically refreshed settings may enable the convergence to jump out of local search of the solution. 
In Section \ref{sec:impact}, we present more details regarding CG and GMRES with lossy checkpointing.
In the following discussion, we always use CG and GMRES to denote the restarted CG and GMRES, respectively, in the context of lossy checkpointing. For these restarted iterative methods, the only dynamic variable we need to checkpoint is the approximate solution vector $x$. 
As shown in Section \ref{sec:checkpoint}, however, even checkpointing one dynamic vector will still lead to a severe performance issue for current or future HPC systems.

\subsection{Performance Model of Lossy Checkpointing}
\label{sec:lossy-perf-model}

In this subsection, we build a performance model for the lossy checkpointing scheme, which is fundamental for analyzing the lossy checkpointing performance theoretically. Based on this performance model, we further derive a sufficient condition, an upper bound of the extra number of iterations caused by lossy data (i.e., Equation (\ref{eq:nbound})), for guaranteeing the performance improvement of the lossy checkpointing scheme. 
Building the performance model requires a few more parameters, as listed in Table 2.

\begin{table}[h]
\centering
\caption{Notations used in the lossy checkpointing performance model}
\vspace{-2mm}
\resizebox{\hsize}{!}{%
\begin{tabular}{|l|l|}
\hline
$T_{comp}$        & Mean time of performing lossy compression                                                         \\ \hline
$T_{decomp}$      & Mean time of performing lossy decompression                                                       \\ \hline
$T_{ckp}^{trad}$  & Mean time of performing one traditional checkpoint                                                \\ \hline
% $T_{ckp}^{lossy}$ & \begin{tabular}[c]{@{}l@{}}The mean time to perform a lossy compressed\\ checkpoint\end{tabular} \\ \hline
$T_{ckp}^{lossy}$              & Mean time of performing a lossy checkpointing                                                     \\ \hline
$T_{overhead}^{lossyCR}$              & Time overhead of performing lossy checkpoint/recovery                                                     \\ \hline
$N'$              & Mean number of extra iterations caused by per lossy recovery                                                              \\ \hline
\end{tabular}
}
\vspace{-2mm}
\end{table}

Since lossy compression introduces errors in the reconstructed dynamic variable(s), the solver may suffer from a delay to converge.
Suppose one recovery will cause extra $N'$ iterations to the convergence on average. Then the total execution time can be rewritten as
\begin{equation}
\label{eq:lossy-ckpt-model}
T_{t} = NT_{it} + T_{ckp}^{lossy}\frac{N}{k} + \frac{T_{t}}{T_{f}}(N' T_{it} + T_{rc}^{lossy} + T_{rb}),
\end{equation}
because  lossy checkpointing needs to perform one decompression during each recovery,  
%lossy checkpointing needs to perform one compression during each checkpoint,
and each recovery will delay $N'$ iterations on average.
Note that $T_{ckp}^{lossy}$ and $T_{rc}^{lossy}$ include the compression time $T_{comp}$ and decompression time $T_{decomp}$, respectively. 
%Also, $T_{ckp}^{lossy}/T_{rc}^{lossy}$ include $T_{comp}/T_{decomp}$ and the time of writing/reading data.
According to \cite{sz17, sz16, zfp}, $T_{comp}$ and $T_{decomp}$ are usually stable for a fixed compression accuracy.

Although the checkpointing/restarting time may differ across various iterations because of different data sizes due to various compression ratios, most  well-known iterative methods can converge quickly such that the value of each element in the approximate solution changes little in the following execution. Hence, the checkpointing data and its size will not change dramatically after several initial iterations, and $T_{ckp}^{lossy}$ and $T_{rc}^{lossy}$ can be assumed to be independent of iterations without loss of generality.

Similar to Section \ref{sec:checkpoint}, we can derive the expected execution time with lossy checkpointing as
\begin{equation*}
\vspace{-2mm}
T_{t} = \frac{NT_{it}}{1 - \sqrt{2\lambda T_{ckp}^{lossy}} - \lambda T_{rc}^{lossy} - \lambda N' T_{it}}
\end{equation*}
and the expected performance overhead of lossy checkpointing as
\begin{equation}
\label{eq:lossy-overhead-ori}
T_{overhead}^{lossyCR} = NT_{it}\cdot \frac{\sqrt{2\lambda T_{ckp}^{lossy}} + \lambda T_{rc}^{lossy} + \lambda N' T_{it}}{1 - \sqrt{2\lambda T_{ckp}^{lossy}} - \lambda T_{rc}^{lossy} - \lambda N' T_{it}}.
\end{equation}
Similarly, we can use $T_{ckp}^{lossy}$ to approximate $T_{rc}^{lossy}$ and simplify the performance overhead formula to 
\begin{equation}
\label{eq:lossy-overhead}
T_{overhead}^{lossyCR} \approx NT_{it}\cdot \frac{\sqrt{2\lambda T_{ckp}^{lossy}} + \lambda T_{ckp}^{lossy} + \lambda N' T_{it}}{1 - \sqrt{2\lambda T_{ckp}^{lossy}} - \lambda T_{ckp}^{lossy} - \lambda N' T_{it}}.
\end{equation}

Now, we can derive a sufficient condition for iterative methods such that the lossy checkpointing scheme  with a lossy compressor is able to obtain a performance gain over the traditional checkpointing scheme without lossy compression techniques.
%Inequality (\ref{eq:nbound}) is a sufficient condition to achieve performance gain when running the iterative methods in the lossy checkpointing scheme integrated with a lossy compressor against the traditional checkpointing scheme that writes/reads original data. 
\begin{theorem}
Denote $\lambda$ and $T_{it}$ by the expected failure rate and expected execution time of an iteration, respectively.
The lossy checkpointing scheme will improve the execution performance for an iterative method as long as the following inequality holds. 
\begin{equation}
\label{eq:nbound}
\begin{array}{l}
N' \leq %F(T_{ckp}^{trad},T_{ckp}^{lossy}, \lambda, T_{it}).
(f(T_{ckp}^{trad},\lambda) - f(T_{ckp}^{trad},\lambda)) / (\lambda T_{it}),\\
where \hspace{1mm} f(t, \lambda) = \sqrt{2\lambda t} + \lambda t
\end{array}
\end{equation}
\end{theorem}
\begin{proof}
To have the lossy checkpointing overhead be lower than that of  traditional checkpointing, we make Equation (\ref{eq:lossy-overhead}) smaller than Equation (\ref{eq:lossless-overhead}):
\begin{equation*}
\resizebox{.9\hsize}{!}{%
$\frac{\sqrt{2\lambda T_{ckp}^{lossy}} + \lambda T_{ckp}^{lossy} + \lambda N' T_{it}}{1 - \sqrt{2\lambda T_{ckp}^{lossy}} - \lambda T_{ckp}^{lossy} - \lambda N' T_{it}} \leq
\frac{\sqrt{2\lambda T_{ckp}^{trad}} + \lambda T_{ckp}^{trad}}{1 - \sqrt{2\lambda T_{ckp}^{trad}} - \lambda T_{ckp}^{trad}}$.
}
\end{equation*}

Further simplifying this inequality, we can get the following formula with respect to the upper bound of $N'$.
\begin{equation*}
\resizebox{.76\hsize}{!}{%
$N' \leq \frac{(\sqrt{2\lambda T_{ckp}^{trad}} + \lambda T_{ckp}^{trad}) - (\sqrt{2\lambda T_{ckp}^{lossy}} + \lambda T_{ckp}^{lossy})}{\lambda T_{it}}$
}
\end{equation*}
Rewriting this inequality with $f(t, \lambda) = \sqrt{2\lambda t} + \lambda t$ will lead to Equation (\ref{eq:nbound}).
\end{proof}

%That is, the lossy checkpointing scheme will improve the execution performance for an iterative method, as long as Inequality (\ref{eq:nbound}) holds.

We give an example to explain how to use Theorem 1 in practice. 
Based on our experiments running GMRES on the Bebop cluster with 2,048 cores, we noted that the lossy compression technique can reduce the checkpointing time $T_{ckp}$ from $120$ seconds to $25$ seconds for GMRES with a checkpoint of about $80$ data (details are presented later in Figure \ref{fig:f3}). 
Suppose the MTTI of a system is one hour (i.e., $\lambda = 1/3600$) and that the GMRES algorithm requires $5,875$ iterations with a total of $7,160$ seconds to converge. Then the mean time of one iteration, namely, $T_{it}$, is about $1.2$ seconds.
We can derive the maximum acceptable number of extra iterations to be 500 based on Equation (\ref{eq:nbound}). Hence,  using a lossy checkpointing scheme is worthwhile if one recovery (with compression error introduced by lossy checkpointing) causes an extra $500$ or fewer iterations (about 9\% of total iterations) to converge,


%Assume the lossy checkpointing delays the iterative methods for extra $N'$ iterations, the total time will be modified to 
%\begin{equation*}
%\frac{(N+N')T_{it}}{1 - \sqrt{2\lambda T_{ckp}} - \lambda T_{ckp}}
%\end{equation*}
%
%And the fault tolerance overhead formula will be changed accordingly as follows.
%\begin{equation*}
%NT_{it}\cdot \frac{N'/N+\sqrt{2\lambda T_{ckp}} + \lambda T_{ckp}}{1 - \sqrt{2\lambda T_{ckp}} - \lambda T_{ckp}}
%\end{equation*}
%
%Let $T_{ckp}^{(1)}$ and $T_{ckp}^{(2)}$ to denote one checkpoint time of the original checkpointing and the lossy checkpointing separately.
%Let $O_1$ and $O_2$ to denote the fault-tolerance overhead with $N$ and $N+N'$ iterations separately.
%So
%\begin{align*}
%O_1 &= NT_{it}\cdot \frac{\sqrt{2\lambda T_{ckp}^{(1)}} + \lambda T_{ckp}^{(1)}}{1 - \sqrt{2\lambda T_{ckp}^{(1)}} - \lambda T_{ckp}^{(1)}} \\
%O_2 &= NT_{it}\cdot \frac{N'/N+\sqrt{2\lambda T_{ckp}^{(2)}} + \lambda T_{ckp}^{(2)}}{1 - \sqrt{2\lambda T_{ckp}^{(2)}} - \lambda T_{ckp}^{(2)}}
%\end{align*}
%
%If we still want to keep the fault-tolerance overhead not increased when lossy checkpointing delays the iterative methods for extra $N'$ iterations, the following relation must be maintained.
%\begin{align*}
%O_1 &\geq O_2 \\
%\frac{\sqrt{2\lambda T_{ckp}^{(1)}} + \lambda T_{ckp}^{(1)}}{1 - \sqrt{2\lambda T_{ckp}^{(1)}} - \lambda T_{ckp}^{(1)}} &\geq  \frac{N'/N+\sqrt{2\lambda T_{ckp}^{(2)}} + \lambda T_{ckp}^{(2)}}{1 - \sqrt{2\lambda T_{ckp}^{(2)}} - \lambda T_{ckp}^{(2)}}
%\end{align*}
%
%Then we can get the formula for $N'/N$ as follows.
%\begin{align} \label{eq: boundary}
%\frac{N'}{N} \leq \frac{  (1 - \sqrt{2\lambda T_{ckp}^{(2)}} - \lambda T_{ckp}^{(2)})(\sqrt{2\lambda T_{ckp}^{(1)}} + \lambda T_{ckp}^{(1)})     }{1 - \sqrt{2\lambda T_{ckp}^{(1)}} - \lambda T_{ckp}^{(1)}} \\ 
%- \frac{  (1 - \sqrt{2\lambda T_{ckp}^{(1)}} - \lambda T_{ckp}^{(1)})(\sqrt{2\lambda T_{ckp}^{(2)}} + \lambda T_{ckp}^{(2)})     }{1 - \sqrt{2\lambda T_{ckp}^{(1)}} - \lambda T_{ckp}^{(1)}} \nonumber 
%\end{align}
%
%The above right hand side equation is the boundary to make $O_2 \leq O_1$.
%In other words, if and only if the relative extra iterations (to the original number of iteration) introduced by lossy checkpointing can be bounded by Equation \ref{eq: boundary}, the fault-tolerance overhead will not increase.
%
%
%If we want to keep the fault-tolerance overhead unchanged when lossy compression delays the iterative methods for $N'$ iterations, the following relation must be maintained.
%\begin{equation*}
%\frac{N'/N+\sqrt{2\lambda T_{ckp}^{(2)}} + \lambda T_{ckp}^{(2)}}{1 - \sqrt{2\lambda T_{ckp}^{(2)}} - \lambda T_{ckp}^{(2)}} =  \frac{O_1}{NT_{it}}
%\end{equation*}
%
%That is 
%\begin{equation*}
%\sqrt{2\lambda T_{ckp}^{(2)}} + \lambda T_{ckp}^{(2)}  = \frac{  \frac{O_1}{NT_{it}} - N'/N}{ \frac{O_1}{NT_{it}} + 1}
%\end{equation*}
%
%So we can solve the equation to get the $T_{ckp}^{(2)}$ as follows.
%\begin{align*}
%T_{ckp}^{(2)} & = (\sqrt{(\frac{  \frac{O_1}{NT_{it}} - N'/N}{ \frac{O_1}{NT_{it}} + 1})^2-2} - \sqrt{2})^2/(4\lambda) \\
%T_{ckp}^{(2)} & = (\sqrt{(\frac{  \mu - N'/N}{ \mu + 1})^2-2} - \sqrt{2})^2/(4\lambda)
%\end{align*}
%where $\mu = \frac{\sqrt{2\lambda T_{ckp}^{(1)}} + \lambda T_{ckp}^{(1)}}{1 - \sqrt{2\lambda T_{ckp}^{(1)}} - \lambda T_{ckp}^{(1)}}$.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}





